Optimal Combination of Linear and Spectral Estimators for Generalized Linear Models

We study the problem of recovering an unknown signal $\boldsymbol x$ given measurements obtained from a generalized linear model with a Gaussian sensing matrix. Two popular solutions are based on a linear estimator $\hat{\boldsymbol x}^{\rm L}$ and a spectral estimator $\hat{\boldsymbol x}^{\rm s}$. The former is a data-dependent linear combination of the columns of the measurement matrix, and its analysis is quite simple. The latter is the principal eigenvector of a data-dependent matrix, and a recent line of work has studied its performance. In this paper, we show how to optimally combine $\hat{\boldsymbol x}^{\rm L}$ and $\hat{\boldsymbol x}^{\rm s}$. At the heart of our analysis is the exact characterization of the joint empirical distribution of $(\boldsymbol x, \hat{\boldsymbol x}^{\rm L}, \hat{\boldsymbol x}^{\rm s})$ in the high-dimensional limit. This allows us to compute the Bayes-optimal combination of $\hat{\boldsymbol x}^{\rm L}$ and $\hat{\boldsymbol x}^{\rm s}$, given the limiting distribution of the signal $\boldsymbol x$. When the distribution of the signal is Gaussian, then the Bayes-optimal combination has the form $\theta\hat{\boldsymbol x}^{\rm L}+\hat{\boldsymbol x}^{\rm s}$ and we derive the optimal combination coefficient. In order to establish the limiting distribution of $(\boldsymbol x, \hat{\boldsymbol x}^{\rm L}, \hat{\boldsymbol x}^{\rm s})$, we design and analyze an Approximate Message Passing (AMP) algorithm whose iterates give $\hat{\boldsymbol x}^{\rm L}$ and approach $\hat{\boldsymbol x}^{\rm s}$. Numerical simulations demonstrate the improvement of the proposed combination with respect to the two methods considered separately.

==> proof_combo.tex <==

\section{Proofs for Section \ref{sec:combo}}


\subsection{Proof of Corollary \ref{cor:crosscor}}

For convenience, denote $\bz_L = \begin{bmatrix}\cT_L(y_1) & \cdots & \cT_L(y_n)\end{bmatrix}^\sT$ and 
$\bZ_s = \diag(\cT_s(y_1), \ldots, \cT_s(y_n)).$
% = f(\bA\bx)$ for appropriate function $f:\R^n\rightarrow\R$ (such a function exists because of \eqref{eq:defy}). 
By definition of the linear estimator,
\begin{align}
\langle\bxl, \bxs\rangle = \frac{\sqrt{d}}{n}\inp{\bA^\sT\bz_L}{\bxs} = \frac{\sqrt{d}}{n}\inp{\bz_L}{\bA\bxs},\label{eq:by_lin_def}
\end{align}
and note that $\bz^L$ is a function of $\bA\bx$. Therefore, we can use Theorem \ref{th:W2conv2} to compute the high-dimensional limit of the  inner-product \eqref{eq:by_lin_def} as follows. Recall the definition of the vector $\bpsi=\big(\bI_n-\frac{1}{\lambda_{\delta}^*}\bZ_s\big)\bA\bxs$ in \eqref{eq:psivec_def}. Then, we have
\begin{align}
\langle\bxl, \bxs\rangle &= \frac{\sqrt{d}}{n}\inp{\left(\id_n-\frac{1}{\lambda_{\delta}^*}\bZ_s\right)^{-1}\bz_L}{\left(\id_n-\frac{1}{\lambda_{\delta}^*}\bZ_s\right)\bA\bxs}  =\frac{\sqrt{d}}{n}\inp{\left(\id_n-\frac{1}{\lambda_{\delta}^*}\bZ_s\right)^{-1}\bz_L}{\bpsi} 
\nn\\&=\sqrt{\frac{d}{n}}\cdot\frac{1}{n}\sum_{i\in[n]} \sqrt{n}\psi_i \cdot \frac{\cT_L(y_i)}{1-\frac{1}{\lambda_{\delta}^*}\cT_s(y_i)}\label{eq:tothm}
\end{align}
At this point, we recognize that the terms $\frac{\cT_L(y_i)}{1-\frac{1}{\lambda_{\delta}^*}\cT_s(y_i)},~i\in[n]$ are functions of $\bg=\bA\bx$. Thus, we can use Theorem \ref{th:W2conv2} and the law of large numbers to conclude from \eqref{eq:tothm} that
\begin{align}
\langle\bxl, \bxs\rangle \ras \frac{b}{\sqrt\delta} \cdot\E\left[ \frac{Z_L \cdot G}{1-\frac{1}{\lambda_{\delta}^*} Z_s} \right],
\end{align}
where $b$ is as in \eqref{eq:b_def}.\mm{Need to make sure that the function is PL(2). I am not sure if we need the law of large numbers here.}

To complete the proof of the corollary, recall from \eqref{eq:norm_lin} that $\|\bxl\|_2 \ras \sqrt{\left(\E\left[Z_LG\right]\right)^2 + \frac{\E\left[Z_L^2\right]}{\delta}}$.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Proof of Lemma \ref{lemma:W2conv_combo_jointGaussian}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We organize the proof of the lemma in four steps as follows. For convenience, let 
$$
\bupsilon=\sqrt{d}\frac{\bxl}{\|\bxl\|_2} \quad\text{and}\quad
\bphi=\sqrt{d}\bxs.
$$

\mm{only one step is here}\ct{All steps are in place now}

\begin{enumerate}
    \item[\bf{Step 1}] We show that the joint empirical distribution of $(\x,\bupsilon,\bphi)$ converges in $W_2$ to the law of 
    \begin{align}\label{eq:Step1}
    (X,\rho_LX + W_L,\rho_s X + W_s)
    \end{align}
     where $W_L\sim\Nn(0,1-\rho_L^2)$ and $W_s\sim\Nn(0,1-\rho_s^2)$ are Gaussians independent of $X$. At this step, we are not specifying neither the correlation nor the  joint distribution of $W_L$ and $W_s$.
    \item[\bf{Step 2}] Using step 1 and Corollary \ref{cor:crosscor}, we compute the correlation $\E[W_LW_s]$.
    \item[\bf{Step 3}] We prove that $W_L$ and $W_s$ are jointly Gaussian.
     \item[\bf{Step 4}] We put things together to complete the proof of the lemma.
\end{enumerate}

\noindent{\bf Step 1.~} The claim is equivalent to showing that, for any $f:\mathbb R^3\to \mathbb R\in {\rm PL}(2)$ and $\Wo_L,\Wo_s$ standard Gaussians independent of $X$, almost surely
\begin{equation}\label{eq:2show_PK}
\lim_{d\to \infty}\left| \frac{1}{d}\sum_{i=1}^d f(\upsilon_i,\varphi_i,x_i) - \mathbb E\{f(\rho_LX+\sqrt{1-\rho_L^2}\Wo_L,\rho_sX+\sqrt{1-\rho_s^2}\Wo_s,X)\} \right|=0.
\end{equation} 
Let $\bR\in \mathbb R^{d \times d}$ be an orthogonal matrix such that $\bR \bx = \bx$. Then, 
\begin{equation}\label{eq:rot_inv_app}
\langle \bx, \ba_i\rangle =\langle \bR \bx, \bR\ba_i \rangle = \langle \bx, \bR\ba_i\rangle .
\end{equation}
Consequently, we have that
\begin{equation}
\bR\bD_n \bR^{\sT}  \stackrel{\mathclap{\text{d}}}{=}\bD_n \quad\text{and}\quad \bR\bA^\sT\bz_L\stackrel{\mathclap{\text{d}}}{=}\bA^\sT\bz_L,
\end{equation}
which immediately implies that
\begin{equation}\label{eq:Rphi}
\bR\bphi  \stackrel{\mathclap{\text{d}}}{=}\bphi\qquad\text{and}\qquad \bR\bupsilon  \stackrel{\mathclap{\text{d}}}{=}\bupsilon.
\end{equation}
Thus,
we can decompose $\bupsilon$ as
% \begin{subequations}\label{eq:dectbphi}
\begin{align}
\bupsilon &= c_d\frac{\sqrt{d}}{\|\bx\|_2} \, \bx + \sqrt{1-c_d^2}\, \bupsilon^{\perp}\quad\text{and}\quad
\bphi = a_d\frac{\sqrt{d}}{\|\bx\|_2} \, \bx + \sqrt{1-a_d^2}\, \bphi^{\perp},\nn
\end{align}
% \end{subequations}
where $\bupsilon^\perp$ and $\bphi^\perp$ are uniformly distributed over the set of vectors orthogonal to $\bx$ with norm $\sqrt{d}$, and also,
$$
 c_d= \left \< \frac{\bx}{\|\bx\|_2},  \frac{\bupsilon}{\sqrt{d}} \right \> \quad\text{and}\quad a_d= \left \< \frac{\bx}{\|\bx\|_2},  \frac{\bphi}{\sqrt{d}} \right \> 
$$
Relating the uniform distribution on the sphere to the normal distribution \cite[Sec.~3.3.3]{vershynin2018high}, we can express $\bupsilon^\perp$ and $\bphi^\perp$ as follows:
\begin{align}
\bupsilon^{\perp} &=\sqrt{d} \,  \frac{\bwo_L - \displaystyle\frac{1}{d}\langle \bwo_L, \bx \rangle \bx}{\Big\|\bwo_L - \displaystyle\frac{1}{d}\langle \bwo_L, \bx\rangle \bx\Big\|_2},\quad\text{$\bwo_L\sim \normal(\b0_d, \bI_d)$ and independent of $\bx$},\nn \\
%
\bphi^{\perp} &=\sqrt{d} \,  \frac{\bwo_s - \displaystyle\frac{1}{d}\langle \bwo_s, \bx\rangle \bx}{\Big\|\bwo_s - \displaystyle\frac{1}{d}\langle \bwo_s, \bx\rangle \bx\Big\|_2},\quad\text{$\bwo_s\sim \normal(\b0_d, \bI_d)$ and independent of $\bx$}\nn.
\end{align}
By the law of large numbers, we have the almost sure limits
\begin{equation}\label{eq:asconv}
\begin{split}
\lim_{d\to\infty}\frac{1}{d}\langle \bwo_L, \bx\rangle = \lim_{d\to\infty}\frac{1}{d}\langle \bwo_s, \bx\rangle &= 0,\\ 
\lim_{d\to\infty}\frac{1}{d}\Big\|\bh - \displaystyle\frac{1}{d}\langle \bwo_L, \bx\rangle \bx\Big\|_2^2=\lim_{d\to\infty}\frac{1}{d}\Big\|\bwo_s - \displaystyle\frac{1}{d}\langle \bwo_s, \bx\rangle \bx\Big\|_2^2 &= 1. 
\end{split}
\end{equation}
Thus, almost surely
$
\lim_{d\to\infty}\frac{1}{d}\|\bupsilon^{\perp} \, - \, \bwo_L \|_2^2 = 0, 
$ and $
\lim_{d\to\infty}\frac{1}{d}\|\bphi^{\perp} \, - \, \bwo_s \|_2^2 = 0.
$
Moreover, from Lemmas \ref{lemma:pt_lin} and \ref{lemma:pt} we have that 
\begin{align}\nn
\lim_{d\to \infty} c_d &= \lim_{d\to \infty} \inp{\frac{\bx}{\norm{\bx}_2}}{\frac{\bxl}{\|{\bxl}\|_2}} =  \rho_L. \nn \\
\lim_{d\to \infty} a_d &= \lim_{d\to \infty} \inp{\frac{\bx}{\norm{\bx}_2}}{{\bxs}} =  \rho_s.\nn
\end{align}
Combining the above and also using the fact that almost surely $\lim_{d\to\infty}\|\bx\|_2/\sqrt{d} = 1$, we find that almost surely
\begin{equation}\label{eq:norm_conv_23}
\lim_{d\to\infty}\frac{1}{d}\left\|\bupsilon - \left(\rho_L \, \bx+\sqrt{1-\rho_L^2}\bwo_L\right)\right\|_2^2 = 0 \quad\text{and}\quad
\lim_{d\to\infty}\frac{1}{d}\left\|\bphi - \left(\rho_s \, \bx+\sqrt{1-\rho_s^2}\bwo_s\right)\right\|_2^2 = 0. 
\end{equation}

We are now ready to prove \eqref{eq:2show_PK}. Note that
\begin{equation}\label{eq:lim23}
\begin{split}
&\left| \frac{1}{d}\sum_{i=1}^d f(\upsilon_i,\varphi_i, x_i) - \frac{1}{d}\sum_{i=1}^d f(\rho_L x_i  + \sqrt{1-\rho_L^2}(\wo_L)_i,\rho_s x_i  + \sqrt{1-\rho_s^2} (\wo_s)_i, x_i) \right| \\
&\qquad\le  \frac{1}{d}\sum_{i=1}^d \left|f(\upsilon_i,\varphi_i, x_i) -  f(\rho_L x_i  + \sqrt{1-\rho_L^2}(\wo_L)_i,\rho_s x_i  + \sqrt{1-\rho_s^2} (\wo_s)_i, x_i) \right|\\
&\le \frac{L}{d}\sum_{i=1}^d\Big\{ \sqrt{|\upsilon_i-(\rho_Lx_i  + \sqrt{1-\rho_L^2}(\wo_L)_i)|^2+|\varphi_i-(\rho_sx_i  + \sqrt{1-\rho_s^2}(\wo_s)_i)|^2} 
\\&\qquad\times \left(1+\sqrt{\upsilon^2+\varphi_i^2+x_i^2}+\sqrt{(\rho_Lx_i  + \sqrt{1-\rho_L^2}(\wo_L)_i)^2+(\rho_sx_i  + \sqrt{1-\rho_s^2}(\wo_s)_i)^2+x_i^2}\right)\,\Big\}\\
&\le L\,\sqrt{\frac{1}{d}\|\bupsilon - (\rho_L \bx+\sqrt{1-\rho_L^2}\bwo_L)\|_2^2+\frac{1}{d}\|\bphi - (\rho_s \bx+\sqrt{1-\rho_s^2}\bwo_s)\|_2^2} \\
&\qquad\times\left(1+\frac{\sqrt{\|\bupsilon\|_2^2+\|\bphi\|_2^2+\|\bx\|_2^2}}{\sqrt{d}}+\frac{\sqrt{\|\rho_L \bx+\sqrt{1-\rho_L^2}\bwo_L\|_2^2+\|\rho_s \bx+\sqrt{1-\rho_s^2}\bwo_s\|_2^2+\|\bx\|_2^2}}{\sqrt{d}}\right),
\end{split}
\end{equation}
where in the second inequality we use that $f\in {\rm PL}(2)$ and in the last inequality we apply Cauchy-Schwarz inequality. Next, we take the limit $d\rightarrow\infty$ in \eqref{eq:lim23}. The first term vanishes by using \eqref{eq:norm_conv_23}. For the second term

By using \eqref{eq:norm_conv_23} in \eqref{eq:lim23}, we deduce that almost surely
\begin{equation}
\lim_{d\to\infty} \left| \frac{1}{d}\sum_{i=1}^d f(\upsilon_i,\varphi_i, x_i) - \frac{1}{d}\sum_{i=1}^d f(\rho_Lx_i  + \sqrt{1-\rho_L^2}(\wo_L)_i,\rho_sx_i  + \sqrt{1-\rho_s^2}(\wo_s)_i, x_i) \right| = 0.
\end{equation}

% To continue, consider (sequence) of functions $\phi_d:(\R^p)^3$ 
% $$
% \phi_d(\rho_L\bx) = \E_{\bwo_L,\bwo_s}\left[ \frac{1}{d}\sum_{i=1}^d f(\rho_Lx_i  + \sqrt{1-\rho_L^2}(\wo_L)_i,\rho_sx_i  + \sqrt{1-\rho_s^2}(\wo_s)_i, x_i)  \right]
% $$


The proof is concluded by applying the law of large numbers to the sum $\frac{1}{d}\sum_{i=1}^d f(\rho_Lx_i  + \sqrt{1-\rho_L^2}(\wo_L)_i,\rho_sx_i  + \sqrt{1-\rho_s^2}(\wo_s)_i, x_i)$.\mm{this works only if the components $x_i$ are independent (or almost so, like for the uniform distribution over the sphere)\ct{Agreed}}

\noindent\textbf{Step 2.}~ On the one hand, from the result of Step 1 (see \eqref{eq:Step1}), we know that 
\begin{align}
    \frac{1}{d}\inp{\bupsilon}{\bphi} &\rP \E\left[(\rho_LX+W_L)(\rho_sX+W_s)\right] \\
    &\qquad= \rho_L\rho_s + \E[W_LW_s],
\end{align}
where we used the fact that $W_L,W_s$ are independent of $X$ and $\E[X^2]=1$.
On the other hand, from Corollary \ref{cor:crosscor}, we know that
\begin{align}
    \frac{1}{d}\inp{\bupsilon}{\bphi} = \inp{\frac{\bxl}{\|\bxl\|_2}}{\bxs} \ras q.
\end{align}
Combining the above displays shows that
\begin{align}
    E[W_LW_s] = {q-\rho_L\rho_s}. \nn    
\end{align}

\noindent\textbf{Step 3.}~Here, we prove that $W_L$ and $W_s$ in \eqref{eq:Step1} are jointly Gaussians. It suffices to show that for any constants $\alpha,\beta\in\R$, the random variable $c_LW_L+c_sW_s$ is Gaussian. We show this as follows.  First, from the convergence result of Step 1, we have that the empirical distribution of the vector 
\begin{align}
    \label{eq:ba_def}
    \ba:=c_L \bupsilon + c_s \bphi - (c_L\rho_L+c_s\rho_s)\x
\end{align}
converges almost surely in $W_2$ to the law of 
\begin{align}
    \label{eq:firstlaw}
    c_LW_L+c_sW_s.
\end{align}

Second, in Lemma \ref{lemma:W2conv_combo} below we compute the limiting law of $x$ and $c_L\bupsilon+c_s\bphi$ as follows. 

\begin{lemma}\label{lemma:W2conv_combo}
Consider the the same setting and the notation of Corollary \ref{cor:crosscor}. Assume that the empirical distribution of $\bx$ converges in the $W_2$ metric to a limiting distribution $P_X$ with unit second moment. Fix arbitrary $c_L,c_s\in\R$ and consider the random vector $\bchi:= c_L \sqrt{d}\frac{\bxl}{\|\bxl\|_2} + c_s \sqrt{d}\bxs$. Then, 
the joint empirical distribution of $\bx$  and $\bchi$  converges almost surely in $W_2$ to the law of 
\begin{equation}\label{eq:joint3}
(X, \zeta X+\sqrt{\xi^2-\zeta^2}W_0),
\end{equation}
where  $W_0\sim\Nn(0,1)$ is independent of $X$ and we defined
\begin{align*}
    \zeta&:=\zeta(c_L,c_s) = c_L\rho_L + c_s \rho_s,\\
    \xi&:=\xi(c_L,c_s) = \sqrt{c_L^2 + c_s^2+2c_Lc_s q}.
\end{align*}
\end{lemma}
The proof of the lemma is very similar to Step 1 above, but is given below for completeness. Before that, let us show how the lemma allows us to complete Step 3. Indeed, the lemma shows that the empirical distribution of the vector $\ba$ in \eqref{eq:ba_def} converges almost surely in $W_2$ to the law of $\sqrt{\xi^2-\zeta^2}W_0$, where $W_0\sim\Nn(0,1)$. Combining this with the limiting law in \eqref{eq:firstlaw}, shows that $c_LW_L+c_sW_s\sim\Nn(0,\xi^2-\zeta^2)$. This completes the proof of Step 3.

\vp
\noindent\textbf{Step 4.}~We put together the results of Steps 1,2 and 3, to complete the proof of Lemma \ref{lemma:W2conv_combo_jointGaussian}. First, from Step 3, $W_L$ and $W_s$ are jointly Gaussian. Second, from Step 2, we know that $\E[W_LW_s] = q-\rho_L\rho_s$. These, together with the convergence result of Step 1 conclude the proof.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Proof of Lemma \ref{lemma:W2conv_combo}}
The proof is similar to the proof in Step 1 above and we frequently refer to it to avoid unnecessary repetitions.  
 Recall the notation $\bphi=\sqrt{d}\bxs$, $\bupsilon=\sqrt{d}\frac{\bxl}{\norm{\bxl}_2}$ and $\bchi=c_L\bupsilon + c_s\bphi$. The claim is equivalent to showing that, for any $f:\mathbb R^2\to \mathbb R\in {\rm PL}(2)$, almost surely
\begin{equation}
\lim_{d\to \infty}\left| \frac{1}{d}\sum_{i=1}^d f(\chi_i,x_i) - \mathbb E\{f(\zeta X+\sqrt{\xi^2-\zeta^2}W_0, X)\} \right|=0.
\end{equation} 

Let $\bR\in \mathbb R^{d \times d}$ be an orthogonal matrix such that $\bR \bx = \bx$. 
% Then, 
% \begin{equation}\label{eq:rot_inv_app}
% \langle \bx, \ba_i\rangle =\langle \bR \bx, \bR\ba_i \rangle = \langle \bx, \bR\ba_i\rangle .
% \end{equation}
% Consequently, we have that
% \begin{equation}
% \bR\bD_n \bR^{\sT}  \stackrel{\mathclap{\text{d}}}{=}\bD_n, \quad\text{and}\quad \bR\bA^\sT\bz_L\stackrel{\mathclap{\text{d}}}{=}\bA^\sT\bz_L,
% \end{equation}
% which immediately implies that
% \begin{equation}
% \bR\bphi  \stackrel{\mathclap{\text{d}}}{=}\bphi\qquad\text{and}\qquad \bR\bupsilon  \stackrel{\mathclap{\text{d}}}{=}\bupsilon.
% \end{equation}
Then, from \eqref{eq:Rphi}, it follows that $\bR\bchi  \stackrel{\mathclap{\text{d}}}{=}\bchi$. Thus, we can decompose $\bchi$ as follows
\begin{align}\nn
    \bchi = \zeta_d \frac{\sqrt{d}}{\|\bx\|_2} \, \bx + \sqrt{\xi_d^2-\zeta_d^2}\, \bchi^{\perp},
\end{align}
where
$
    \xi_d^2 = \frac{\norm{\bchi}_2^2}{d}, 
$
$\bchi^{\perp}$ is uniformly distributed over the set of vectors orthogonal to $\bx$ with norm $\sqrt{d}$ and
\begin{equation}\nn
 \left \< \frac{\bx}{\|\bx\|_2},  \frac{\bchi}{\sqrt{d}} \right \> =  \zeta_d.
\end{equation}
Consequently, we can write $\bchi^{\perp}$ as
\begin{align}\label{eq:decbphi}
\bchi^{\perp} &= \sqrt{d} \,  \frac{\bu - \displaystyle\frac{1}{d}\langle \bh, \bx\rangle \bx}{\Big\|\bh - \displaystyle\frac{1}{d}\langle \bh, \bx\rangle \bx\Big\|_2},
\end{align}
where $\bh\sim \normal(\b0_d, \bI_d)$ and independent of $\bx$. Similar to \eqref{eq:asconv}, we may then conclude that
% By the law of large numbers, we have the almost sure limits
% \begin{equation}
% \begin{split}
% \lim_{d\to\infty}\frac{1}{d}\langle \bh, \bx\rangle &= 0,\\ 
% \lim_{d\to\infty}\frac{1}{d}\Big\|\bh - \displaystyle\frac{1}{d}\langle \bh, \bx\rangle \bx\Big\|_2^2 &= 1. 
% \end{split}
% \end{equation}
% Thus, we conclude that 
almost surely
\begin{equation}\label{eq:limxperp}
\lim_{d\to\infty}\frac{1}{d}\|\bchi^{\perp} \, - \, \bh \|_2^2 = 0,
\end{equation}
which, by using also \eqref{eq:decbphi}, implies that 
\begin{equation}\label{eq:lim0}
\lim_{d\to\infty}\frac{1}{d}\left\|\bchi - \left(\zeta_d \frac{\sqrt{d}}{\|\bx\|_2}\bx+\sqrt{\xi_d^2-\zeta_d^2} \, \bh\right)\right\|_2^2 = 0.
\end{equation}

Next, we compute the limits of the coefficients $\zeta_d$ and $\xi_d$. First, by Lemmas \ref{lemma:pt_lin} and \ref{lemma:pt}, we have that
\begin{equation}\label{eq:lemmalim}
\begin{split}
\lim_{d\to \infty} \zeta_d &= c_L \,\lim_{d\to \infty}\left \< \frac{\bx}{\|\bx\|_2},  \frac{\bxl}{\norm{\bxl}_2} \right \>+c_s \,\lim_{d\to \infty}\left \< \frac{\bx}{\|\bx\|_2},  \bxs \right \> = c_L\rho_L + c_s\rho_s =: \zeta.
\end{split}
\end{equation}
Second, by Corollary \ref{cor:crosscor}, we have that
\begin{align}
    \lim_{d\to \infty} \xi_d^2 = c_L^2 + c_s^2 + 2\,c_L \, c_s\,\lim_{d\to \infty} \left \< \frac{\bxl}{\|\bxl\|_2},  \bxs \right \> = c_L^2 + c_s^2 + 2\,c_L \, c_s\,q =: \xi^2, 
\end{align}
where $q$ is defined in \eqref{eq:crosscorr}.
 Furthermore, $\|\bx\|_2=\sqrt{d}$. Combining these leads to
\begin{equation}\label{eq:lim1}
\lim_{d\to\infty}\frac{1}{d}\left\|\bchi - \left(\zeta\bx+\sqrt{\xi^2-\zeta^2}\bh\right)\right\|_2^2 = 0.
\end{equation}


Next, note that
\begin{equation}\label{eq:lim2}
\begin{split}
\left| \frac{1}{d}\sum_{i=1}^d f(\chi_i, x_i) - \frac{1}{d}\sum_{i=1}^d f(\zeta x_i  + \sqrt{\xi^2-\zeta^2}h_i, x_i) \right| &\le  \frac{1}{d}\sum_{i=1}^d \left|f(\chi_i, x_i) -  f(\zeta x_i  + \sqrt{\xi^2-\zeta^2}h_i, x_i) \right|\\
&\hspace{-17em}\le \frac{L}{d}\sum_{i=1}^d |\chi_i-(\zeta x_i  + \sqrt{\xi^2-\zeta^2}h_i)| \left(1+\sqrt{\chi_i^2+x_i^2}+\sqrt{(\zeta x_i  + \sqrt{\xi^2-\zeta^2}h_i)^2+x_i^2}\right)\\
&\hspace{-17em}\le L\frac{\|\bchi - (\zeta  \bx+\sqrt{\xi^2-\zeta^2}\bh)\|_2}{\sqrt{d}} \left(1+\frac{\sqrt{\|\bchi\|_2^2+\|\bx\|_2^2}}{\sqrt{d}}+\frac{\sqrt{\|\zeta \bx+\sqrt{\xi^2-\zeta^2}\bh\|_2^2+\|\bx\|_2^2}}{\sqrt{d}}\right),
\end{split}
\end{equation}
where in the second line we use that $f\in {\rm PL}(2)$ and in the third line we apply Cauchy-Schwarz inequality. By combining \eqref{eq:lim1} and \eqref{eq:lim2}, we deduce that almost surely
\begin{equation}
\lim_{d\to\infty} \left| \frac{1}{d}\sum_{i=1}^d f(\chi_i, x_i) - \frac{1}{d}\sum_{i=1}^d f(\zeta x_i  + \sqrt{\xi^2-\zeta^2}h_i, x_i) \right| = 0.
\end{equation}
The proof is concluded by applying the law of large numbers to the sum $d^{-1}\sum_{i=1}^d f(\zeta x_i  + \sqrt{\xi^2-\zeta^2}h_i, x_i)$.\ct{Same remark as the end of the proof of Step 1}

